Label-aware Hard Negative Sampling Strategies with Momentum Contrastive Learning for Implicit Hate Speech Detection

Detecting implicit hate speech that is not directly hateful remains a challenge. Recent research has attempted to detect implicit hate speech by applying contrastive learning to pre-trained language models such as BERT and RoBERTa, but the proposed models still do not have a significant advantage over cross-entropy loss-based learning. We found that contrastive learning based on randomly sampled batch data does not encourage the model to learn hard negative samples. In this work, we propose Label-aware Hard Negative sampling strategies (LAHN) that encourage the model to learn detailed features from hard negative samples, instead of naive negative samples in random batch, using momentum-integrated contrastive learning. LAHN outperforms the existing models for implicit hate speech detection both in- and cross-datasets. The code is available at https://github.com/Hanyang-HCC-Lab/LAHN

==> Tables/Table_1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Table 1}
\label{table_1}
% \setlength\tabcolsep{2.7pt}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|c|c|l|ccc|c}
\hline
\multirow{2}{*}{\textbf{Dataset}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pre-trained \\ Language Model\end{tabular}} &
  \multirow{2}{*}{\textbf{External knowledge}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} &
  \multicolumn{3}{c|}{\textbf{Evaluation Dataset}} &
  \multirow{2}{*}{\textbf{Average}} \\ \cline{5-7}
 &
   &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{\textbf{IHC}} &
  \multicolumn{1}{l|}{\textbf{SBIC}} &
  \multicolumn{1}{l|}{\textbf{DynaHate}} &
   \\ \hline
\multirow{12}{*}{IHC} & \multirow{6}{*}{BERT-base}    & \multirow{4}{*}{X} & CE           &                &                &                &                \\
                      &                               &                    & Gunel et al  &                &                &                &                \\
                      &                               &                    & Suresh et al &                &                &                &                \\
                      &                               &                    & Ours         &                &                &                &                \\ \cline{3-8} 
                      &                               & \multirow{2}{*}{O} & Kim et al    &                &                &                &                \\
                      &                               &                    & Ours         &                &                &                &                \\ \cline{2-8} 
                      & \multirow{6}{*}{RoBERTa-base} & \multirow{4}{*}{X} & CE           & 80.06          & 53.78          & 46.49          & 60.11          \\
                      &                               &                    & Gunel et al  & 78.60          & 57.77          & 46.68          & 61.01          \\
                      &                               &                    & Suresh et al &                &                &                &                \\
                      &                               &                    & Ours         & 80.12          & 58.55          & \textbf{47.64} & \textbf{62.10} \\ \cline{3-8} 
                      &                               & \multirow{2}{*}{O} & Kim et al    & 79.29          & \textbf{59.23} & 47.48          & 62.0           \\
                      &                               &                    & Ours         & \textbf{80.65} & 57.56          & 47.01          & 61.74          \\ \hline
\end{tabular}
}
\end{table*}


==> Tables/Table_1_2_BAK.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Table 1}
\label{table_1}
% \setlength\tabcolsep{2.7pt}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{c|c|c|l|cccc|c}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Training} \\ \textbf{Dataset}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Pre-trained} \\ \textbf{Language Model}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{External} \\ \textbf{Knowledge}\end{tabular}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} &
  \multicolumn{4}{c|}{\textbf{Evaluation Dataset}} &
  \multirow{2}{*}{\textbf{Average}} \\ \cline{5-8}
 &
   &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{\textbf{IHC}} &
  \multicolumn{1}{l|}{\textbf{SBIC}} &
  \multicolumn{1}{l|}{\textbf{DynaHate}} &
  \multicolumn{1}{l|}{\textbf{ToxiGen}} &
   \\ \hline
\multirow{12}{*}{IHC} & \multirow{7}{*}{BERT-base}    & X & CE           & 77.49          & 57.05          & 53.69     &  60.80   & 62.26          \\
                      &                               & X & UCL (et al)  & 71.66          & 53.14          & 52.82     &  54.88   & 58.13          \\
                      &                               & X & SCL (et al)  & 77.81          & 57.21          & 55.21     &  59.74   & 62.49          \\
                      % &                               &                    & LCL (et al) &                &                &         &    1   &                \\
                      &                               & X & \textbf{Ours}& \textbf{78.40}  & \textbf{62.51} & \textbf{57.47}  &  \textbf{62.29}   &\textbf{65.17}          \\ \cline{3-9} 
                      &                               & O & ImpCon (et al)    &  74.39   & 54.55  & \textbf{59.41}  &   59.64    & 62.00            \\
                      &       & O & \textbf{Ours}& \textbf{78.62}    & \textbf{58.45}    & 52.95    &   \textbf{61.49}   & \textbf{62.88}   \\ \cline{2-9} \hhline{~-=======}
                      & \multirow{7}{*}{RoBERTa-base} & X & CE           & 79.95          & 55.03          & 47.34     & 59.35     & 60.42\         \\
                      &                               & X & UCL (et al)  & 71.37   & \textbf{60.19}   & \textbf{52.92}   & 56.17  & 60.16          \\
                      &                               & X & SCL (et al)  & 79.33          & 56.86       & 46.40   & \textbf{60.56}    & \textbf{60.79}          \\
                      % &                               &                    & LCL (et al) &                &                &          & 1     &                \\
                      &                               & X & \textbf{Ours}& \textbf{80.11}  & 54.76  & 46.68  & 57.46  & 59.75 \\ \cline{3-9} 
                      &                               & O & ImpCon (et al)    & 78.78     & 63.82          & 50.13    & 60.81      & \textbf{63.39}           \\
                      &                               & O & \textbf{Ours}& \textbf{80.58} & 60.09 & 48.62 & \textbf{63.94} & 63.31          \\ \hline
\end{tabular}
}

\vspace{0.05cm}

\resizebox{0.95\textwidth}{!}{
\begin{tabular}{c|c|c|l|cccc|c}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Training} \\ \textbf{Dataset}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Pre-trained} \\ \textbf{Language Model}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{External} \\ \textbf{Knowledge}\end{tabular}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} &
  \multicolumn{4}{c|}{\textbf{Evaluation Dataset}} &
  \multirow{2}{*}{\textbf{Average}} \\ \cline{5-8}
 &
   &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{\textbf{IHC}} &
  \multicolumn{1}{l|}{\textbf{SBIC}} &
  \multicolumn{1}{l|}{\textbf{DynaHate}} &
  \multicolumn{1}{l|}{\textbf{ToxiGen}} &
   \\ \hline
\multirow{12}{*}{SBIC} & \multirow{6}{*}{BERT-base}    & X & CE        & 59.47    & 83.72     & 60.17    &  67.54  & 67.73          \\
                       &                               & X & UCL (et al)  & 58.21     & 81.56    & 59.24  &  64.68  & 65.92          \\
                       &                               & X & SCL (et al)  & 59.96   & \textbf{84.14}   & \textbf{60.97} & 67.62   & 68.17          \\
                       % &                               &                    & LCL (et al) &                &                &        &        &                \\
                       &                               & X & \textbf{Ours}& \textbf{61.51}          & 83.98          & 60.27     &  \textbf{68.68}   & \textbf{68.61}          \\ \cline{3-9} 
                       &                               & O & ImpCon (et al)& 58.34         & 83.53          & \textbf{59.36}      &  66.41  & 66.91   \\
                       &                               & O & \textbf{Ours}& \textbf{60.60}          & \textbf{84.31}          & 58.21     &  \textbf{68.11}   & \textbf{67.81}          \\ \cline{2-9} \hhline{~-=======}
                       & \multirow{6}{*}{RoBERTa-base} & X & CE           & 59.68          & 85.27 & 61.62     &  68.54   & 68.78          \\
                       &                               & X & UCL (et al)  & 57.65          & 81.82 & 58.53     &  65.96   & 65.99          \\
                       &                               & X & SCL (et al)  & 57.90          & 85.25 & 61.17     &  67.92   & 68.06          \\
                       % &                               &                    & LCL (et al) &                &      &          &      &                \\
                       &                               & X & \textbf{Ours}& \textbf{61.13} & \textbf{85.45} & \textbf{63.20} &  \textbf{69.07}   & \textbf{69.71} \\ \cline{3-9} 
                       &                               & O & ImpCon (et al)    & 56.23 & 84.66 & 60.70     & 66.40    &  67.00         \\
                       &                               & O & \textbf{Ours}& \textbf{61.00} & \textbf{85.80} & \textbf{61.63}    &   \textbf{68.72}   & \textbf{69.29} \\ \hline
\end{tabular}
}

\end{table*}






% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \caption{Table 1}
% \label{table_1}
% % \setlength\tabcolsep{2.7pt}
% \resizebox{0.95\textwidth}{!}{
% \begin{tabular}{c|c|c|l|cccc|c}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Training} \\ \textbf{Dataset}\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Pre-trained} \\ \textbf{Language Model}\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{External} \\ \textbf{Knowledge}\end{tabular}} &
%   \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} &
%   \multicolumn{4}{c|}{\textbf{Evaluation Dataset}} &
%   \multirow{2}{*}{\textbf{Average}} \\ \cline{5-8}
%  &
%    &
%    &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{l|}{\textbf{IHC}} &
%   \multicolumn{1}{l|}{\textbf{SBIC}} &
%   \multicolumn{1}{l|}{\textbf{DynaHate}} &
%   \multicolumn{1}{l|}{\textbf{ToxiGen}} &
%    \\ \hline
% \multirow{12}{*}{IHC} & \multirow{7}{*}{BERT-base}    & \multirow{4}{*}{X} & CE           & 77.49          & 57.05          & 53.69     &  60.80   & 62.26          \\
%                       &                               &                    & UCL (et al)  & 71.66          & 53.14          & 52.82     &  54.88   & 58.13          \\
%                       &                               &                    & SCL (et al)  & 77.81          & 57.21          & 55.21     &  59.74   & 62.49          \\
%                       % &                               &                    & LCL (et al) &                &                &         &    1   &                \\
%                       &                               &      & \textbf{Ours}& \textbf{78.40}  & \textbf{62.51} & \textbf{57.47}  &  \textbf{62.29}   &\textbf{65.17}          \\ \cline{3-9} 
%                       &                               & \multirow{2}{*}{O} & ImpCon (et al)    &  74.39   & 54.55  & \textbf{59.41}  &   59.64    & 62.00            \\
%                       &       &   & \textbf{Ours}& \textbf{78.62}    & \textbf{58.45}    & 52.95    &   \textbf{61.49}   & \textbf{62.88}   \\ \cline{2-9} \hhline{~-=======}
%                       & \multirow{7}{*}{RoBERTa-base} & \multirow{4}{*}{X} & CE           & 79.95          & 55.03          & 47.34     & 59.35     & 60.42\         \\
%                       &                               &                    & UCL (et al)  & 71.37   & \textbf{60.19}   & \textbf{52.92}   & 56.17  & 60.16          \\
%                       &                               &                    & SCL (et al)  & 79.33          & 56.86       & 46.40   & \textbf{60.56}    & \textbf{60.79}          \\
%                       % &                               &                    & LCL (et al) &                &                &          & 1     &                \\
%                       &                               &                    & \textbf{Ours}& \textbf{80.11}  & 54.76  & 46.68  & 57.46  & 59.75 \\ \cline{3-9} 
%                       &                               & \multirow{2}{*}{O} & ImpCon (et al)    & 78.78     & 63.82          & 50.13    & 60.81      & \textbf{63.39}           \\
%                       &                               &       & \textbf{Ours}& \textbf{80.58} & 60.09 & 48.62 & \textbf{63.94} & 63.31          \\ \hline
% \end{tabular}
% }

% \vspace{0.05cm}

% \resizebox{0.95\textwidth}{!}{
% \begin{tabular}{c|c|c|l|cccc|c}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Training} \\ \textbf{Dataset}\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Pre-trained} \\ \textbf{Language Model}\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{External} \\ \textbf{Knowledge}\end{tabular}} &
%   \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} &
%   \multicolumn{4}{c|}{\textbf{Evaluation Dataset}} &
%   \multirow{2}{*}{\textbf{Average}} \\ \cline{5-8}
%  &
%    &
%    &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{l|}{\textbf{IHC}} &
%   \multicolumn{1}{l|}{\textbf{SBIC}} &
%   \multicolumn{1}{l|}{\textbf{DynaHate}} &
%   \multicolumn{1}{l|}{\textbf{ToxiGen}} &
%    \\ \hline
% \multirow{12}{*}{SBIC} & \multirow{6}{*}{BERT-base}    & \multirow{4}{*}{X} & CE        & 59.47    & 83.72     & 60.17    &  67.54  & 67.73          \\
%                        &                               &                    & UCL (et al)  & 58.21     & 81.56    & 59.24  &  64.68  & 65.92          \\
%                        &                               &                    & SCL (et al)  & 59.96   & \textbf{84.14}   & \textbf{60.97} & 67.62   & 68.17          \\
%                        % &                               &                    & LCL (et al) &                &                &        &        &                \\
%                        &                               &                    & \textbf{Ours}& \textbf{61.51}          & 83.98          & 60.27     &  \textbf{68.68}   & \textbf{68.61}          \\ \cline{3-9} 
%                        &                               & \multirow{2}{*}{O} & ImpCon (et al)& 58.34         & 83.53          & \textbf{59.36}      &  66.41  & 66.91   \\
%                        &                               &                    & \textbf{Ours}& \textbf{60.60}          & \textbf{84.31}          & 58.21     &  \textbf{68.11}   & \textbf{67.81}          \\ \cline{2-9} \hhline{~-=======}
%                        & \multirow{6}{*}{RoBERTa-base} & \multirow{4}{*}{X} & CE           & 59.68          & 85.27 & 61.62     &  68.54   & 68.78          \\
%                        &                               &                    & UCL (et al)  & 57.65          & 81.82 & 58.53     &  65.96   & 65.99          \\
%                        &                               &                    & SCL (et al)  & 57.90          & 85.25 & 61.17     &  67.92   & 68.06          \\
%                        % &                               &                    & LCL (et al) &                &      &          &      &                \\
%                        &                               &                    & \textbf{Ours}& \textbf{61.13} & \textbf{85.45} & \textbf{63.20} &  \textbf{69.07}   & \textbf{69.71} \\ \cline{3-9} 
%                        &                               & \multirow{2}{*}{O} & ImpCon (et al)    & 56.23 & 84.66 & 60.70     & 66.40    &  67.00         \\
%                        &                               &                    & \textbf{Ours}& \textbf{61.00} & \textbf{85.80} & \textbf{61.63}    &   \textbf{68.72}   & \textbf{69.29} \\ \hline
% \end{tabular}
% }

% \end{table*}






% SBIC Toxigen 추가 전 보존용
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{c|c|c|l|ccc|c}
% \hline
% \multirow{2}{*}{\textbf{Dataset}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Pre-trained} \\ \textbf{Language Model}\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{External} \\ \textbf{Knowledge}\end{tabular}} &
%   \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} &
%   \multicolumn{3}{c|}{\textbf{Evaluation Dataset}} &
%   \multirow{2}{*}{\textbf{Average}} \\ \cline{5-7}
%  &
%    &
%    &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{l|}{\textbf{IHC}} &
%   \multicolumn{1}{l|}{\textbf{SBIC}} &
%   \multicolumn{1}{l|}{\textbf{DynaHate}} &
%    \\ \hline
% \multirow{12}{*}{SBIC} & \multirow{6}{*}{BERT-base}    & \multirow{4}{*}{X} & CE           & 59.47          & 83.72          & 60.17          & 67.79          \\
%                        &                               &                    & UCL (et al)  & 58.21          & 81.56          & 59.24          & 66.34          \\
%                        &                               &                    & SCL (et al)  & 59.96          & 84.14          & 60.97          & 68.36          \\
%                        &                               &                    & LCL (et al) &                &                &                &                \\
%                        &                               &                    & \textbf{Ours}& 61.51          & 83.98          & 60.27          & 68.59          \\ \cline{3-8} 
%                        &                               & \multirow{2}{*}{O} & ImpCon (et al)& 58.34         & 83.53          & \textbf{59.36}          & 67.08                \\
%                        &                               &                    & \textbf{Ours}& \textbf{60.60}          & \textbf{84.31}          & 58.21          & \textbf{67.71}          \\ \cline{2-8} \hhline{~-======}
%                        & \multirow{6}{*}{RoBERTa-base} & \multirow{4}{*}{X} & CE           & 59.68          & 85.27          & 61.62          & 68.86          \\
%                        &                               &                    & UCL (et al)  & 57.65          & 81.82          & 58.53          & 66.00          \\
%                        &                               &                    & SCL (et al)  & 57.90          & 85.25          & 61.17          & 68.11          \\
%                        &                               &                    & LCL (et al) &                &                &                &                \\
%                        &                               &                    & \textbf{Ours}& \textbf{61.13}          & \textbf{85.45}          & \textbf{63.20} & \textbf{69.93} \\ \cline{3-8} 
%                        &                               & \multirow{2}{*}{O} & ImpCon (et al)    & 56.23          & 84.66 & 60.70          &  67.20         \\
%                        &                               &                    & \textbf{Ours}& \textbf{61.00} & \textbf{85.80} & \textbf{61.63}          & \textbf{69.48} \\ \hline
% \end{tabular}
% }

% \end{table*}


==> Tables/Table_1_2_BAK_latest.tex <==
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\bluecheck}{{\color{blue}\cmark}}
\newcommand{\redxmark}{{\color{red}\xmark}}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{To investigate both case with/without external knowledge, we employ two datasets (IHC, SBIC) with implication information as the training dataset among the public benchmark dataset. The top table shows the results of the in-dataset (IHC) evaluation and the cross-dataset (SBIC, DynaHate, ToxiGen) evaluation. The bottom table contains the results of the in-dataset (SBIC) evaluation and the cross-dataset (IHC, DynaHate, ToxiGen) evaluation.}
\label{table_1}
% \setlength\tabcolsep{2.7pt}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{c|c|c|l|cccc|c}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Training} \\ \textbf{Dataset}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Pre-trained} \\ \textbf{Language Model}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{External} \\ \textbf{Knowledge}\end{tabular}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} &
  \multicolumn{4}{c|}{\textbf{Evaluation Dataset}} &
  \multirow{2}{*}{\textbf{Average}} \\ \cline{5-8}
 &
   &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{\textbf{IHC}} &
  \multicolumn{1}{l|}{\textbf{SBIC}} &
  \multicolumn{1}{l|}{\textbf{DynaHate}} &
  \multicolumn{1}{l|}{\textbf{ToxiGen}} &
   \\ \hline
\multirow{12}{*}{IHC} & \multirow{7}{*}{BERT-base}    & \xmark & Cross-Entropy Loss (CE)           & 77.49          & 57.05          & 53.69     &  60.80   & 62.26          \\
                      % &                               & X & UCL (et al)  & 71.66          & 53.14          & 52.82     &  54.88   & 58.13          \\
                      &                               & \xmark & SCL~\cite{gunel2020supervised}  & 77.81          & 59.19          & 55.84     &  62.19   & 63.76          \\
                      % &                               & \xmark & LCL~\cite{suresh2021not}  &  77.45   &   60.67   & 57.72  &  61.66  & 64.38          \\
                      % &                               &                    & LCL (et al) &                &                &         &    1   &                \\
                      &                               & \xmark & \textbf{LAHN (ours)}& \textbf{78.40}  & \textbf{62.83} & \textbf{57.80}  &  \textbf{63.21}   &\textbf{65.56}          \\ \cline{3-9} 
                      &                               & \cmark & ImpCon~\cite{kim2022generalizable}    &  78.39   & 54.55  & \textbf{59.41}  &   59.64    & 63.00            \\
                      &       & \cmark & \textbf{LAHN (ours)}& \textbf{78.62}    & \textbf{62.02}    & 56.13    &   \textbf{62.92}   & \textbf{64.92}   \\ \cline{2-9} \hhline{~-=======}
                      & \multirow{7}{*}{RoBERTa-base} & \xmark & Cross-Entropy Loss (CE)           & 79.95          & 55.03          & 47.34     & 59.35     & 60.42\         \\
                      % &                               & X & UCL (et al)  & 71.37   & \textbf{60.19}   & \textbf{52.92}   & 56.17  & 60.16          \\
                      &                               & \xmark & SCL~\cite{gunel2020supervised}  & 79.33          & 57.77       & 46.92   & 60.89    & 61.23          \\
                      % &                               & \xmark & LCL~\cite{suresh2021not}  & 79.78       & 60.46 & \textbf{48.51}  &  \textbf{65.32}   & \textbf{63.52}          \\
                      % &                               &                    & LCL (et al) &                &                &          & 1     &                \\
                      &                               & \xmark & \textbf{LAHN (ours)}& \textbf{80.11}  & \textbf{60.57}  & \textbf{48.46}  & \textbf{63.94}  & \textbf{63.27} \\ \cline{3-9} 
                      &                               & \cmark & ImpCon~\cite{kim2022generalizable}    & 78.78     & 63.82          & \textbf{50.13}    & 61.79   & 63.63           \\
                      &                               & \cmark & \textbf{LAHN (ours)}& \textbf{80.58} & \textbf{64.01} & 49.54 & \textbf{64.49} & \textbf{64.66}          \\ \hline
\end{tabular}
}

\vspace{0.05cm}

\resizebox{0.95\textwidth}{!}{
\begin{tabular}{c|c|c|l|cccc|c}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Training} \\ \textbf{Dataset}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Pre-trained} \\ \textbf{Language Model}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{External} \\ \textbf{Knowledge}\end{tabular}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} &
  \multicolumn{4}{c|}{\textbf{Evaluation Dataset}} &
  \multirow{2}{*}{\textbf{Average}} \\ \cline{5-8}
 &
   &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{\textbf{IHC}} &
  \multicolumn{1}{l|}{\textbf{SBIC}} &
  \multicolumn{1}{l|}{\textbf{DynaHate}} &
  \multicolumn{1}{l|}{\textbf{ToxiGen}} &
   \\ \hline
\multirow{12}{*}{SBIC} & \multirow{6}{*}{BERT-base}    & \xmark & Cross-Entropy Loss (CE)        & 59.47    & 83.72     & 60.17    &  67.54  & 67.73          \\
                       % &                               & X & UCL (et al)  & 58.21     & 81.56    & 59.24  &  64.68  & 65.92          \\
                       &                               & \xmark & SCL~\cite{gunel2020supervised}  & 60.07   & \textbf{84.14}   & 60.97 & 67.62   & 68.20          \\
                       % &                               & \xmark & LCL~\cite{suresh2021not}  & -          & 83.90          & -     &  -   & -          \\
                       % &                               &                    & LCL (et al) &                &                &        &        &                \\
                       &                               & \xmark & \textbf{LAHN (ours)}& \textbf{62.36}          & 83.98          & \textbf{63.06}     &  \textbf{69.58}   & \textbf{69.75}          \\ \cline{3-9} 
                       &                               & \cmark & ImpCon~\cite{kim2022generalizable} & 58.64         & 83.53          & 59.50      &  66.54  & 67.05   \\
                       &                               & \cmark & \textbf{LAHN (ours)}& \textbf{61.58}          & \textbf{84.31}          & \textbf{60.97}     &  \textbf{68.52}   & \textbf{68.85}          \\ \cline{2-9} \hhline{~-=======}
                       & \multirow{6}{*}{RoBERTa-base} & \xmark & Cross-Entropy Loss (CE)           & 59.68          & 85.27 & 61.62     &  68.54   & 68.78          \\
                       % &                               & X & UCL (et al)  & 57.65          & 81.82 & 58.53     &  65.96   & 65.99          \\
                       &                               & \xmark & SCL~\cite{gunel2020supervised}  & 59.61          & 85.25 & 61.17     &  68.77   & 68.70          \\
                       % &                               & \xmark & LCL~\cite{suresh2021not}  & -          & 84.81          & -     &  -   & -          \\
                       % &                               &                    & LCL (et al) &                &      &          &      &                \\
                       &                               & \xmark & \textbf{LAHN (ours)}& \textbf{64.74} & \textbf{85.45} & \textbf{64.32} &  \textbf{70.61}   & \textbf{71.28} \\ \cline{3-9} 
                       &                               & \cmark & ImpCon~\cite{kim2022generalizable} & 56.95 & 84.66 & 60.70     & 66.77    &  67.27         \\
                       &                               & \cmark & \textbf{LAHN (ours)}& \textbf{64.05} & \textbf{85.80} & \textbf{63.26}    &   \textbf{69.91}   & \textbf{70.76} \\ \hline
\end{tabular}
}

\end{table*}






% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \caption{Table 1}
% \label{table_1}
% % \setlength\tabcolsep{2.7pt}
% \resizebox{0.95\textwidth}{!}{
% \begin{tabular}{c|c|c|l|cccc|c}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Training} \\ \textbf{Dataset}\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Pre-trained} \\ \textbf{Language Model}\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{External} \\ \textbf{Knowledge}\end{tabular}} &
%   \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} &
%   \multicolumn{4}{c|}{\textbf{Evaluation Dataset}} &
%   \multirow{2}{*}{\textbf{Average}} \\ \cline{5-8}
%  &
%    &
%    &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{l|}{\textbf{IHC}} &
%   \multicolumn{1}{l|}{\textbf{SBIC}} &
%   \multicolumn{1}{l|}{\textbf{DynaHate}} &
%   \multicolumn{1}{l|}{\textbf{ToxiGen}} &
%    \\ \hline
% \multirow{12}{*}{IHC} & \multirow{7}{*}{BERT-base}    & \multirow{4}{*}{X} & CE           & 77.49          & 57.05          & 53.69     &  60.80   & 62.26          \\
%                       &                               &                    & UCL (et al)  & 71.66          & 53.14          & 52.82     &  54.88   & 58.13          \\
%                       &                               &                    & SCL (et al)  & 77.81          & 57.21          & 55.21     &  59.74   & 62.49          \\
%                       % &                               &                    & LCL (et al) &                &                &         &    1   &                \\
%                       &                               &      & \textbf{Ours}& \textbf{78.40}  & \textbf{62.51} & \textbf{57.47}  &  \textbf{62.29}   &\textbf{65.17}          \\ \cline{3-9} 
%                       &                               & \multirow{2}{*}{O} & ImpCon (et al)    &  74.39   & 54.55  & \textbf{59.41}  &   59.64    & 62.00            \\
%                       &       &   & \textbf{Ours}& \textbf{78.62}    & \textbf{58.45}    & 52.95    &   \textbf{61.49}   & \textbf{62.88}   \\ \cline{2-9} \hhline{~-=======}
%                       & \multirow{7}{*}{RoBERTa-base} & \multirow{4}{*}{X} & CE           & 79.95          & 55.03          & 47.34     & 59.35     & 60.42\         \\
%                       &                               &                    & UCL (et al)  & 71.37   & \textbf{60.19}   & \textbf{52.92}   & 56.17  & 60.16          \\
%                       &                               &                    & SCL (et al)  & 79.33          & 56.86       & 46.40   & \textbf{60.56}    & \textbf{60.79}          \\
%                       % &                               &                    & LCL (et al) &                &                &          & 1     &                \\
%                       &                               &                    & \textbf{Ours}& \textbf{80.11}  & 54.76  & 46.68  & 57.46  & 59.75 \\ \cline{3-9} 
%                       &                               & \multirow{2}{*}{O} & ImpCon (et al)    & 78.78     & 63.82          & 50.13    & 60.81      & \textbf{63.39}           \\
%                       &                               &       & \textbf{Ours}& \textbf{80.58} & 60.09 & 48.62 & \textbf{63.94} & 63.31          \\ \hline
% \end{tabular}
% }

% \vspace{0.05cm}

% \resizebox{0.95\textwidth}{!}{
% \begin{tabular}{c|c|c|l|cccc|c}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Training} \\ \textbf{Dataset}\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Pre-trained} \\ \textbf{Language Model}\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{External} \\ \textbf{Knowledge}\end{tabular}} &
%   \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} &
%   \multicolumn{4}{c|}{\textbf{Evaluation Dataset}} &
%   \multirow{2}{*}{\textbf{Average}} \\ \cline{5-8}
%  &
%    &
%    &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{l|}{\textbf{IHC}} &
%   \multicolumn{1}{l|}{\textbf{SBIC}} &
%   \multicolumn{1}{l|}{\textbf{DynaHate}} &
%   \multicolumn{1}{l|}{\textbf{ToxiGen}} &
%    \\ \hline
% \multirow{12}{*}{SBIC} & \multirow{6}{*}{BERT-base}    & \multirow{4}{*}{X} & CE        & 59.47    & 83.72     & 60.17    &  67.54  & 67.73          \\
%                        &                               &                    & UCL (et al)  & 58.21     & 81.56    & 59.24  &  64.68  & 65.92          \\
%                        &                               &                    & SCL (et al)  & 59.96   & \textbf{84.14}   & \textbf{60.97} & 67.62   & 68.17          \\
%                        % &                               &                    & LCL (et al) &                &                &        &        &                \\
%                        &                               &                    & \textbf{Ours}& \textbf{61.51}          & 83.98          & 60.27     &  \textbf{68.68}   & \textbf{68.61}          \\ \cline{3-9} 
%                        &                               & \multirow{2}{*}{O} & ImpCon (et al)& 58.34         & 83.53          & \textbf{59.36}      &  66.41  & 66.91   \\
%                        &                               &                    & \textbf{Ours}& \textbf{60.60}          & \textbf{84.31}          & 58.21     &  \textbf{68.11}   & \textbf{67.81}          \\ \cline{2-9} \hhline{~-=======}
%                        & \multirow{6}{*}{RoBERTa-base} & \multirow{4}{*}{X} & CE           & 59.68          & 85.27 & 61.62     &  68.54   & 68.78          \\
%                        &                               &                    & UCL (et al)  & 57.65          & 81.82 & 58.53     &  65.96   & 65.99          \\
%                        &                               &                    & SCL (et al)  & 57.90          & 85.25 & 61.17     &  67.92   & 68.06          \\
%                        % &                               &                    & LCL (et al) &                &      &          &      &                \\
%                        &                               &                    & \textbf{Ours}& \textbf{61.13} & \textbf{85.45} & \textbf{63.20} &  \textbf{69.07}   & \textbf{69.71} \\ \cline{3-9} 
%                        &                               & \multirow{2}{*}{O} & ImpCon (et al)    & 56.23 & 84.66 & 60.70     & 66.40    &  67.00         \\
%                        &                               &                    & \textbf{Ours}& \textbf{61.00} & \textbf{85.80} & \textbf{61.63}    &   \textbf{68.72}   & \textbf{69.29} \\ \hline
% \end{tabular}
% }

% \end{table*}






% SBIC Toxigen 추가 전 보존용
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{c|c|c|l|ccc|c}
% \hline
% \multirow{2}{*}{\textbf{Dataset}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Pre-trained} \\ \textbf{Language Model}\end{tabular}} &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{External} \\ \textbf{Knowledge}\end{tabular}} &
%   \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} &
%   \multicolumn{3}{c|}{\textbf{Evaluation Dataset}} &
%   \multirow{2}{*}{\textbf{Average}} \\ \cline{5-7}
%  &
%    &
%    &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{l|}{\textbf{IHC}} &
%   \multicolumn{1}{l|}{\textbf{SBIC}} &
%   \multicolumn{1}{l|}{\textbf{DynaHate}} &
%    \\ \hline
% \multirow{12}{*}{SBIC} & \multirow{6}{*}{BERT-base}    & \multirow{4}{*}{X} & CE           & 59.47          & 83.72          & 60.17          & 67.79          \\
%                        &                               &                    & UCL (et al)  & 58.21          & 81.56          & 59.24          & 66.34          \\
%                        &                               &                    & SCL (et al)  & 59.96          & 84.14          & 60.97          & 68.36          \\
%                        &                               &                    & LCL (et al) &                &                &                &                \\
%                        &                               &                    & \textbf{Ours}& 61.51          & 83.98          & 60.27          & 68.59          \\ \cline{3-8} 
%                        &                               & \multirow{2}{*}{O} & ImpCon (et al)& 58.34         & 83.53          & \textbf{59.36}          & 67.08                \\
%                        &                               &                    & \textbf{Ours}& \textbf{60.60}          & \textbf{84.31}          & 58.21          & \textbf{67.71}          \\ \cline{2-8} \hhline{~-======}
%                        & \multirow{6}{*}{RoBERTa-base} & \multirow{4}{*}{X} & CE           & 59.68          & 85.27          & 61.62          & 68.86          \\
%                        &                               &                    & UCL (et al)  & 57.65          & 81.82          & 58.53          & 66.00          \\
%                        &                               &                    & SCL (et al)  & 57.90          & 85.25          & 61.17          & 68.11          \\
%                        &                               &                    & LCL (et al) &                &                &                &                \\
%                        &                               &                    & \textbf{Ours}& \textbf{61.13}          & \textbf{85.45}          & \textbf{63.20} & \textbf{69.93} \\ \cline{3-8} 
%                        &                               & \multirow{2}{*}{O} & ImpCon (et al)    & 56.23          & 84.66 & 60.70          &  67.20         \\
%                        &                               &                    & \textbf{Ours}& \textbf{61.00} & \textbf{85.80} & \textbf{61.63}          & \textbf{69.48} \\ \hline
% \end{tabular}
% }

% \end{table*}


==> Tables/Table_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Table 2}
\label{table_2}
% \setlength\tabcolsep{2.7pt}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{c|c|c|l|ccc|c}
\hline
\multirow{2}{*}{\textbf{Dataset}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pre-trained \\ Language Model\end{tabular}} &
  \multirow{2}{*}{\textbf{External knowledge}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Objective}}} &
  \multicolumn{3}{c|}{\textbf{Evaluation Dataset}} &
  \multirow{2}{*}{\textbf{Average}} \\ \cline{5-7}
 &
   &
   &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{l|}{\textbf{IHC}} &
  \multicolumn{1}{l|}{\textbf{SBIC}} &
  \multicolumn{1}{l|}{\textbf{DynaHate}} &
   \\ \hline
\multirow{12}{*}{SBIC} & \multirow{6}{*}{BERT-base}    & \multirow{4}{*}{X} & CE           &                &                &                &                \\
                       &                               &                    & Gunel et al  &                &                &                &                \\
                       &                               &                    & Suresh et al &                &                &                &                \\
                       &                               &                    & Ours         &                &                &                &                \\ \cline{3-8} 
                       &                               & \multirow{2}{*}{O} & Kim et al    &                &                &                &                \\
                       &                               &                    & Ours         &                &                &                &                \\ \cline{2-8} 
                       & \multirow{6}{*}{RoBERTa-base} & \multirow{4}{*}{X} & CE           & 60.02          & 85.12          & 61.81          & 68.98          \\
                       &                               &                    & Gunel et al  & 59.61          & 84.76          & 60.19          & 68.19          \\
                       &                               &                    & Suresh et al &                &                &                &                \\
                       &                               &                    & Ours         & 60.43          & 85.17          & \textbf{62.79} & \textbf{69.46} \\ \cline{3-8} 
                       &                               & \multirow{2}{*}{O} & Kim et al    & 59.42          & \textbf{85.38} & 62.02          & 68.94          \\
                       &                               &                    & Ours         & \textbf{60.98} & \textbf{85.75} & 61.79          & \textbf{69.51} \\ \hline
\end{tabular}
}
\end{table*}
